Your browsing behavior for a Big Mac: Economics of Personal Information Online

Most online services (Google, Facebook etc.) operate by providing a service to users for free, and in return they collect and monetize personal information (PI) of the users. This operational model is inherently economic, as the "good" being traded and monetized is PI. This model is coming under increased scrutiny as online services are moving to capture more PI of users, raising serious privacy concerns. However, little is known on how users valuate different types of PI while being online, as well as the perceptions of users with regards to exploitation of their PI by online service providers. In this paper, we study how users valuate different types of PI while being online, while capturing the context by relying on Experience Sampling. We were able to extract the monetary value that 168 participants put on different pieces of PI. We find that users value their PI related to their offline identities more (3 times) than their browsing behavior. Users also value information pertaining to financial transactions and social network interactions more than activities like search and shopping. We also found that while users are overwhelmingly in favor of exchanging their PI in return for improved online services, they are uncomfortable if these same providers monetize their PI.

==> plugin.tex <==
Data Collection
To monitor browsing behavior, record answers to experience sampling questions, and record bids to auctions, we developed a Firefox plugin and webserver.
In order to keep track of users, each user was assigned a unique id.
Whenever a new webpage loaded, the plugin recorded the user id, url, access time, and IP address.  
In order to determine the category of the website a user was viewing, we created a database mapping domain names to categories.  
To this end, we used the website Alexa.com.
For websites not included in Alexa.com, we used the categorization software created for Adnostic.
During the auction and experience sampling portion of the study, we would periodically ask users for bids pertaining to each category.
A pop-up would appear on the screen, displaying a question for a specific type of auction.  
Users would have to enter something for this auction before continuing browsing.
During the experience sampling portion of the survey, several pop-ups in succession would appear a few times a day.
Users would have to select multiple choice responses before continuing their browsing.
The three types of information (browsing information, auction bids, and experience sampling response) were sent at regular intervals to a central server, which aggregated results.

